New Results on Online Resource Minimization

We consider the online resource minimization problem in which jobs with hard deadlines arrive online over time at their release dates. The task is to determine a feasible schedule on a minimum number of machines. We rigorously study this problem and derive various algorithms with small constant competitive ratios for interesting restricted problem variants. As the most important special case, we consider scheduling jobs with agreeable deadlines. We provide the first constant ratio competitive algorithm for the non-preemptive setting, which is of particular interest with regard to the known strong lower bound of n for the general problem. For the preemptive setting, we show that the natural algorithm LLF achieves a constant ratio for agreeable jobs, while for general jobs it has a lower bound of Omega(n^(1/3)). We also give an O(log n)-competitive algorithm for the general preemptive problem, which improves upon the known O(p_max/p_min)-competitive algorithm. Our algorithm maintains a dynamic partition of the job set into loose and tight jobs and schedules each (temporal) subset individually on separate sets of machines. The key is a characterization of how the decrease in the relative laxity of jobs influences the optimum number of machines. To achieve this we derive a compact expression of the optimum value, which might be of independent interest. We complement the general algorithmic result by showing lower bounds that rule out that other known algorithms may yield a similar performance guarantee.

==> intro.tex <==
\section{Introduction} Minimizing the resource usage is a key  to the
achievement of economic, environmental or societal goals.
%
%workspace procurement, electricity consumption, where
%the controllable portion of total costs varies with the maximum amount
%of resource procured. 
%
We consider the fundamental problem of minimizing the number of
machines that is necessary for feasibly scheduling jobs with
release dates and hard deadlines. We consider the online variant of this problem in which every job
becomes known to the online algorithm only at its release date. We
denote this problem as {\em online machine minimization problem}. We also
consider a {\em semi-online} variant in which we give the
online algorithm slightly more information by giving the optimal
number of machines as part of the input.

We develop several algorithms for
preemptive and non-preemptive problem variants, and evaluate
their performance by  the competitive ratio, a widely-used measure that
compares the solution value of an online algorithm with an optimal
offline value. We derive the first constant-competitive 
algorithms for certain variants of (semi-)online machine minimization
and improve several others. Our main result is a preemptive $\OO(\log
n)$-competitive algorithm for the most general problem.

\medskip

\noindent {\bf Previous results.} The preemptive semi-online machine minimization problem, in which the
optimal number of machines known in advance, has been
investigated  by Phillips et al.~\cite{phillipsSTW02}. They show a
general lower bound of $\frac{5}{4}$ and leave a huge gap to the
upper bound $\OO(\log \frac{p_{\max}}{p_{\min}})$ on the competitive
ratio for the so-called {\em Least Laxity First} 
(\LLF) Algorithm. Not so surprisingly, they also rule out that the {\em Earliest Deadline
  First} (\EDF) Algorithm could improve on the performance of \LLF;
indeed they show a lower bound of
$\Omega(\frac{p_{\max}}{p_{\min}})$. It is a wide open question if
preemptive (semi-)online machine minimization admits a constant-factor
online algorithm.

The non-preemptive problem is considerably harder than the preemptive
problem. If the set of jobs arrives online over time, then no algorithm
can achieve a constant or even sublinear competitive ratio~\cite{Saha13}. %A lower
%bound of~$\log_3 \frac{p_{\max}}{p_{\min}}$, with $p_{\max}$ and~$p_{\min}$ being the maximum and minimum
 % processing times, respectively, was shown by Saha~\cite{Saha13}. As
  %observed by Devanur et al.~\cite{DevanurMPY14}, the same construction gives also a lower
  %bound of~$n$. 
However, relevant special cases admit
online algorithms with small constant worst-case guarantees. The
problem with unit processing times was studied in a series of
papers~\cite{KleywegtNST99,ShiY08,KaoCRW12,Saha13,DevanurMPY14} and implicitly in
the context of energy-minimization in~\cite{BansalKP07}. It has been shown that an optimal online
algorithm has the exact competitive ratio~$e\approx
2.72$~\cite{BansalKP07,DevanurMPY14}. For non-preemptive scheduling of
jobs with equal deadlines, an upper bound of~$16$ is given
in~\cite{DevanurMPY14}.


% A relaxed variant of our online machine minimization problem has been
% studied %by Kleywegt et al.
% in~\cite{KleywegtNST99}. In our terminology,
% their model allows to process jobs simultaneously on several
% machines. They give algorithms with small constant competitive ratios
% and describe an optimal semi-online algorithm.

Online deadline scheduling with extra speedup is another related
problem variant. We are given the same input as in the semi-online
machine minimization problem. Instead of equipping an online algorithm
with additional machines, the given~$m$ machines may run at an increased
speed~$s\geq 1$. The goal is to find an online scheduling algorithm that requires
minimum speed~$s$.  This problem seems much better understood and
(nearly) tight speedup factors below~$2$ are
known~(see~\cite{phillipsSTW02,lamT99,anandGM11}). However, the power
of speed is much stronger than additional machines since it allows
parallel processing of jobs to some extent. Algorithms that perform
well for the speed-problem, such as, \EDF, \LLF and a deadline-ordered
algorithm, do not admit constant performance guarantees for the
machine minimization problem.

We also mention that the offline problem, in
which all jobs are known in advance, can be solved
optimally in polynomial time if job preemption is allowed~\cite{horn74}. The solution of
the natural linear programming formulation can be rounded in a
straightforward way by assigning fractionally assigned workload in a round robin
fashion over all machines within a time unit. Again, the problem complexity increases drastically if
preemption is not allowed. In fact, the problem of  deciding whether
one machine suffices to schedule all the jobs non-preemptively is strongly
NP-complete~\cite{GareyJ77}. It is even open if a constant-factor
approximation exists; a lower bound of~$2-\eps$ was given
in~\cite{CieliebakEHWW04}. The currently best known non-preemptive approximation algorithm
is by Chuzhoy et al.~\cite{ChuzhoyGKN04} who propose a sophisticated
rounding procedure for a linear
programming relaxation that yields an approximation factor of $\OO(\sqrt{\frac{\log n}{\log\log
    n}})$. Small constant factors were obtained for special
cases~\cite{CieliebakEHWW04,YuZ09}: in particular, Yu and Zhang~\cite{YuZ09}
give a~$2$-approximation when all release dates are equal and
a~$6$-approximation when all processing times are equal.


\medskip
\noindent {\bf Our contribution.} We develop several algorithms and
bounding techniques for the (semi-)online machine minimization
problem. Our main result is a $\OO(\log n)$-competitive algorithm for the general preemptive online
problem. This is the first improvement on a nearly twenty years old $\OO(\log
(p_{\max}/p_{\min}))$-competitive algorithm by Phillips et
al.~\cite{phillipsSTW02,phillipsSTW97}. Their result was actually
obtained for the semi-online problem in which the optimal
number of machines is known in advance. But as we shall see it can be
used to solve the online problem as well. In fact, we show that the
online machine minimization problem can be reduced to the semi-online
problem by losing at most a factor~$4$ in the competitive ratio. This
is true for preemptive as well as non-preemptive~scheduling.

\begin{table}
  \begin{small}
  \definecolor{darkred}{rgb}{0.7,0,0}
  \def\arraystretch{1.15}
  \begin{tabularx}{\linewidth}{@{}cZZZZZZZZ@{}}
    \toprule
    & \multicolumn{4}{ c }{preemptive} & \multicolumn{4}{ c }{non-preemptive} \\
    & \multicolumn{2}{ c }{{\footnotesize \OPT} known} & \multicolumn{2}{ c }{{\footnotesize \OPT}
      unknown} & \multicolumn{2}{ c }{{\footnotesize \OPT} known} & \multicolumn{2}{ c
    }{{\footnotesize \OPT} unknown}\\ 
   & LB & UB & LB & UB & LB & UB & LB & UB\\ 
    \midrule
    general & $\frac{5}{4}$~\cite{phillipsSTW02}
    &\textcolor{darkred}{$\mathcal{O}\left(\log n\right)$} &
    $e$~\cite{BansalKP07,DevanurMPY14}
    &\textcolor{darkred}{$\mathcal{O}\left(\log n\right)^\star$} &
    $n$~\cite{Saha13}  & $-$ & $n$~\cite{Saha13}  & $-$ \\
   
    $p_j \leq \alpha(d_j-r_j)$ & $-$ & \textcolor{darkred}{$\frac{1}{\left(1-\alpha\right)^2}$} & $-$ &
    \textcolor{darkred}{$\frac{4}{\left(1-\alpha\right)^2}^\star$}
    & $n$~\cite{Saha13} & $-$ & $n$~\cite{Saha13} & $-$\\

    agreeable deadlines & $-$ & \textcolor{darkred}{$18$} &
    $e$~\cite{BansalKP07,DevanurMPY14} &\textcolor{darkred}{$72^\star$} & $-$
    & \textcolor{darkred}{$ 8$} & $e$~\cite{BansalKP07,DevanurMPY14} & \textcolor{darkred}{$15$} \\

    $d_j\equiv d$ & $-$ &\textcolor{darkred}{$1$} &
    $e$~\cite{BansalKP07,DevanurMPY14}& \textcolor{darkred}{$4^\star$} & $-$
    & \textcolor{darkred}{$5\frac{1}{4}$} & $e$~\cite{BansalKP07,DevanurMPY14}&\textcolor{darkred}{$11\frac{1}{9}$}\\
  
    $p_j\equiv p$ & \textcolor{darkred}{$\frac{8}{7}$} &
    \textcolor{darkred}{$3$} & $e$~\cite{BansalKP07,DevanurMPY14} &
    \textcolor{darkred}{$9.38$}  & \textcolor{darkred}{$\frac{8}{7}$} & \textcolor{darkred}{$2$}
    &$e$~\cite{BansalKP07,DevanurMPY14}& \textcolor{darkred}{$8^\star$}\\
  
    $p_j\equiv 1$ & $-$ & $1$~\cite{KaoCRW12} & $e$~\cite{BansalKP07,DevanurMPY14} &
    $e$~\cite{BansalKP07,DevanurMPY14} & $-$ & $1$~\cite{KaoCRW12} &
    $e$~\cite{BansalKP07,DevanurMPY14} & $e$~\cite{BansalKP07,DevanurMPY14} \\
  \bottomrule
\end{tabularx}
\caption{State of the art for (semi-)online machine
  minimization. New results presented in this paper are colored red
  (and  have no reference). Results for the online setting that are
  directly derived from the semi-online setting are marked with a
  star~($^\star$). Trivial bounds are excluded ($-$).} 
  \label{tab:results}
  \end{small}
\end{table}

Our main algorithm maintains a dynamic partition of the jobs into
critical and safe jobs and schedules each (temporal) subset
individually on separate sets of machines. The safe jobs are scheduled
by \EDF whereas the critical jobs require a more sophisticated
treatment. The key is a characterization of how the decrease in the
relative laxity of jobs influences the optimum number of machines. To
quantify this we derive  a compact expression of the optimum value,
which might be of independent interest. Then we distribute the
critical jobs evenly over a well-chosen number of machines to keep the
relative laxity sufficiently large. 

In addition to our main algorithmic result we show lower bounds that rule out that other
known algorithms, such as \LLF or any deadline-ordered algorithm, may
yield a similar or even better performance guarantee. Any improvement
requires a more sophisticated approach. 

We also present a rigorous study of interesting restricted problem
variants and show small constant competitive ratios. Here, we include
the non-preemptive problem for which in general strong lower bounds
show that no online algorithm admits a competitive ratio sublinear
in~$n$. With our results we improve on previously known bounds or we give the
first nontrivial results. The special case of {\em agreeable deadlines} could
be seen as the most general class of restricted instances. In this
case, the order of deadlines for all jobs coincides with the order of
their release dates. Here we give the first constant competitive
ratios. They are based on a characterization of tight and loose jobs
which are handled individually. %by known algorithms \EDF and \LLF.
We also quantify how the tightness of jobs influences the performance
of algorithm such as \EDF and \LLF, which might be of independent
interest. Other special cases we consider are jobs with equal
processing times (improving on an earlier result by~\cite{DevanurMPY14}) or with a uniform deadline. A summary of our new results
can be found in Table~\ref{tab:results}.




We remark that our algorithms run in polynomial time (except the non-preemptive online algorithms). As a side
result, we even improve on a previous approximation result for
non-preemptive offline machine minimization when the optimum is not
known. Our semi-online $2$-competitive algorithm for jobs with equal
processing times can be easily turned into an offline~$3$-approximation which
improves upon a known~$6$-approximation~\cite{YuZ09}.

\medskip
\noindent {\em Outline of this paper.} We introduce in Section~\ref{mp-sec:prelim}
some notation and algorithms, and we show a problem reduction from the online problem
to the semi-online problem. In Section~\ref{mp-sec:optimum} we give a compact
representation of the optimum value. Our main result, a preemptive $\OO(\log
n)$-competitive algorithm, is described and analyzed in
Section~\ref{mp-sec:main-alg}. Finally, in
Section~\ref{mp-sec:special-cases} we give first or improved
results for special cases: agreeable deadlines, equal processing times
and uniform deadlines.


%% Local Variables:
%% TeX-master: "paper.tex"
%% End:
